Learned Inertial Odometry for Autonomous Drone Racing

Inertial odometry is an attractive solution to the problem of state estimation for agile quadrotor flight. It is inexpensive, lightweight, and it is not affected by perceptual degradation. However, only relying on the integration of the inertial measurements for state estimation is infeasible. The errors and time-varying biases present in such measurements cause the accumulation of large drift in the pose estimates. Recently, inertial odometry has made significant progress in estimating the motion of pedestrians. State-of-the-art algorithms rely on learning a motion prior that is typical of humans but cannot be transferred to drones. In this work, we propose a learning-based odometry algorithm that uses an inertial measurement unit (IMU) as the only sensor modality for autonomous drone racing tasks. The core idea of our system is to couple a model-based filter, driven by the inertial measurements, with a learning-based module that has access to the thrust measurements. We show that our inertial odometry algorithm is superior to the state-of-the-art filter-based and optimization-based visual-inertial odometry as well as the state-of-the-art learned-inertial odometry in estimating the pose of an autonomous racing drone. Additionally, we show that our system is comparable to a visual-inertial odometry solution that uses a camera and exploits the known gate location and appearance. We believe that the application in autonomous drone racing paves the way for novel research in inertial odometry for agile quadrotor flight.

==> figures/methodology_flowchart.tex <==
\begin{tikzpicture}[>=latex]
\def\h{1cm}
\def\dy{0.2cm}
\def\w{2cm}
\tikzstyle{box} = [rectangle, draw, align = center, inner sep = 0pt, text width = 2cm, minimum height = \h, minimum width = \w]
\tikzstyle{label} = [midway, align=left, inner sep = 0pt]
\tikzstyle{leftlabel} = [label, align=left, inner sep = 0pt, pos = 0, anchor = south west, yshift = 1mm]

\coordinate (left) at (-2.5, 0);
\node at (0,0) (buffer) [box] {Buffer};
\node [minimum width=2cm, minimum height=1.8cm, align=left, text width = 1.7cm, text depth = 1cm, right = 1cm of buffer] (nn) { NN 
\vspace*{1mm}

\tikzset{%
  every neuron/.style={
    circle,
    draw,
    minimum size=0.1cm,
    inner sep=0pt,
  },
}
\begin{tikzpicture}[x=1.5cm, y=1.5cm, >=stealth, yscale=0.1, xscale=0.14]
\foreach \m/\l [count=\y] in {1,...,6}
  \node [every neuron/.try, neuron \m/.try] (input-\m) at (0,3.5-\y) {};
\foreach \m [count=\y] in {1,...,4}
  \node [every neuron/.try, neuron \m/.try ] (hidden1-\m) at (3,2.5-\y) {};
\foreach \m [count=\y] in {1,2}
  \node [every neuron/.try, neuron \m/.try ] (output-\m) at (6,1.5-\y) {};
\foreach \l [count=\i] in {1,...,6}
  \draw [] (input-\i) -- ++(-1,0);
\foreach \i in {1,...,6}
  \foreach \j in {1,...,4}
    \draw [] (input-\i) -- (hidden1-\j);
\foreach \i in {1,...,4}
  \foreach \j in {1,2}
    \draw [] (hidden1-\i) -- (output-\j);
\foreach \l [count=\i] in {1,2}
  \draw [] (output-\i) -- ++(1,0);
\end{tikzpicture}
};
\draw (nn.north west) -- ([yshift=-0.5cm]nn.north east) -- ([yshift=0.5cm]nn.south east) -- (nn.south west) -- cycle ;

\node (imu) [below = 2.5cm of buffer.east, box] {IMU \\ Prop.};
\node (update) [right = 1cm of imu, box] {Update};
\draw [->] (imu) -- coordinate [midway] (ekf) (update);
\node (ekf_box) at ([yshift=0.25cm]ekf) [minimum height = 1.8*\h, minimum width = 6cm, draw] {};
\node at (ekf_box.north west) [anchor=north west]{EKF};

\draw [->] ([yshift=\dy] left |- buffer.west) -- node [leftlabel] {$\mathbf{T}_b$} ([yshift=\dy]buffer.west);
\draw [->] ([yshift=1.5*\dy]ekf_box -| left) -- node [leftlabel] {$\boldsymbol\omega_b$} ([yshift=1.5*\dy]ekf_box.west) coordinate [pos=0.5] (wb);
\draw [->] ([yshift=-1.5*\dy]ekf_box -| left) -- node [leftlabel] {$\mathbf a_b$} ([yshift=-1.5*\dy]ekf_box.west);
\draw [->] (buffer) -- (nn);
\coordinate (buffer_east_pt) at ([xshift=-0.5cm, yshift=-\dy]buffer.west);
\draw [->] (wb -| buffer_east_pt) |- ([yshift=-\dy]buffer.west);
% \draw [->, dashed] ([xshift=-0.2cm]ekf_box.north west -| buffer.south) -| node [label, pos = 0.75, align = center, above left = 1mm and 0.5mm, rotate=90] {$\mathbf v_w$} ([xshift=-0.2cm]buffer.south);
\draw [->] ([xshift=0.4cm]ekf_box.north west -| buffer.south) -| node [label, pos = 0.75, align = center, above left = 1mm and 0.5mm, rotate=90] {$\mathbf{R}^{w}_{b}$} ([xshift=0.4cm]buffer.south);
\draw [->] (nn.east) -| node [label, pos = 0.75, align = center, above left = 1mm and 0.5mm, rotate=90] {$\Delta \mathbf p$} ([xshift=0.5cm] nn.east |- ekf_box.north east);

\node [minimum width=2cm, minimum height=1.8cm, align=center, text width = 1.7cm, text depth = 1cm, right = 1cm of ekf_box, anchor=south west] (drone) {
Quadcopter

\vspace*{2mm}
\begin{tikzpicture}
\def\arm{0.3cm};
\def\r{0.15cm};
\def\rs{\r/1.414};
\draw (\arm, \arm) -- (-\arm, -\arm);
\draw (-\arm, \arm) -- (\arm, -\arm);
\draw (\arm+\rs, \arm+\rs) circle (\r);
\draw (\arm+\rs, -\arm-\rs) circle (\r);
\draw (-\arm-\rs, \arm+\rs) circle (\r);
\draw (-\arm-\rs, -\arm-\rs) circle (\r);
\end{tikzpicture}
\vspace*{1mm}

$\mathbf{R}_{b}^{w}, \mathbf{v}_{b}^{w}, \mathbf{p}_{b}^{w}, \mathbf{b}_{\text{a}}, \mathbf{b}_{\text{g}}$
};

\draw [->] (ekf_box.east) -- (drone.south west);


\end{tikzpicture}

==> sections/acknowledgment.tex <==
\section*{Acknowledgments} \label{sec:Acknowledgments}

==> tex_figures/eyecatcher.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/eyecatcher.png}
    \vspace*{-18pt}
    \caption{By combining a residual neural network in a model-based filter, our method is able to estimate the trajectory of an autonomous racing drone.}
    \label{fig:eyecatcher}
    \vspace*{-12pt}
\end{figure}

==> tex_figures/perceptual_challenges.tex <==
\begin{figure}[t!]
    \centering
    \vspace*{-12pt}
    \includegraphics[width=1\linewidth]{figures/perceptual_challenges.png}
    \vspace*{-18pt}
    \caption{Perceptual challenges in drone racing: low light, motion blur, high dynamic range, and low texture.}\label{fig:perceptual_challenges}
    \vspace*{-24pt}
\end{figure}


==> tex_figures/plot_lemniscate_trans_err.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/lemniscate_reltrans_errs.png}
    % \vspace*{-12pt}
    \caption{Lemniscate trajectory. Relative translation errors achieved by SVO, OpenVINS, TLIO and IMO.}
    % \vspace*{-9pt}
    \label{fig:lemniscate_reltrans_errs}
\end{figure}
